Adaptive Conditional Expert Selection Network for Multi-domain Recommendation

Mixture-of-Experts (MOE) has recently become the de facto standard in Multi-domain recommendation (MDR) due to its powerful expressive ability. However, such MOE-based method typically employs all experts for each instance, leading to scalability issue and low-discriminability between domains and experts. Furthermore, the design of commonly used domain-specific networks exacerbates the scalability issues. To tackle the problems, We propose a novel method named CESAA consists of Conditional Expert Selection (CES) Module and Adaptive Expert Aggregation (AEA) Module to tackle these challenges. Specifically, CES first combines a sparse gating strategy with domain-shared experts. Then AEA utilizes mutual information loss to strengthen the correlations between experts and specific domains, and significantly improve the distinction between experts. As a result, only domain-shared experts and selected domain-specific experts are activated for each instance, striking a balance between computational efficiency and model performance. Experimental results on both public ranking and industrial retrieval datasets verify the effectiveness of our method in MDR tasks.

==> authors.tex <==

% \author{
% {Kuiyao Dong\textsuperscript{1\textasteriskcentered{}},
% Xingyu Lou\textsuperscript{2\textasteriskcentered{}},
% Feng Liu\textsuperscript{1}, Ruian Wang\textsuperscript{1}, Wenyi Yu\textsuperscript{1}, \\ 
% Ping Wang\textsuperscript{1}, Jun Wang\textsuperscript{1†}}
% }
% \authornote{%
% Both authors contributed equally to this research. Yu Yang performed this work as an intern at OPPO
% }
% \authornote{Corresponding author.}

% \def\thefootnote{*}\footnotetext{These authors contributed equally to this work}
% \affiliation{
%   \country{{\textsuperscript{1}OPPO, Shenzhen, China}}
% }
% \affiliation{
%   \country{\textsuperscript{2}Shenzhen International Graduate School, Tsinghua University Shenzhen, China}
% }
% \email{{louxingyu, dongkuiyao, huangheyuan2, yuwenyi, ping.wang}@oppo.com,yu-yang23@mails.singhua.edu.cn,li.xiu@sz.tsinghua.edu.cn,junwang.lu@gmail.com}
